Cooling of Hybrid Stars with Spin Down Compression

We study the cooling of hybrid stars coupling with spin-down. Due to the spin-down of hybrid stars, the interior density continuously increases, different neutrino reactions may be triggered(from the modified Urca process to the quark and nucleon direct Urca process) at different stages of evolution. We calculate the rate of neutrino emissivity of different reactions and simulate the cooling curves of the rotational hybrid stars. The results show the cooling curves of hybrid stars clearly depend on magnetic field if the direct urca reactions occur during the spin-down. Comparing the results of the rotational star model with the transitional static model, we find the cooling behavior of rotational model is more complicated, the temperature of star is higher, especially when direct urca reactions appear in process of rotation. And then we find that the predicted temperatures of some rotating hybrid stars are compatible with the pulsar's data which are contradiction with the results of transitional method.

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
natbib.sty     ---- This package reimplements the LaTeX \cite command
f?.eps         ---- two demo figures used in the LaTeX template source

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org


